Few-shot Unified Question Answering: Tuning Models or Prompts?

Question-answering (QA) tasks often investigate specific question types, knowledge domains, or reasoning skills, leading to specialized models catering to specific categories of QA tasks. While recent research has explored the idea of unified QA models, such models are usually explored for high-resource scenarios and require re-training to extend their capabilities. To overcome these drawbacks, the paper explores the potential of two paradigms of tuning, model, and prompts, for unified QA under a low-resource setting. The paper provides an exhaustive analysis of their applicability using 16 QA datasets, revealing that prompt tuning can perform as well as model tuning in a few-shot setting with a good initialization. The study also shows that parameter-sharing results in superior few-shot performance, simple knowledge transfer techniques for prompt initialization can be effective, and prompt tuning achieves a significant performance boost from pre-training in a low-resource regime. The research offers insights into the advantages and limitations of prompt tuning for unified QA in a few-shot setting, contributing to the development of effective and efficient systems in low-resource scenarios.

==> src/extra.tex <==
%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{Figs/Overall_model_agreement_heatmap.png}
%\vspace*{-2em}
%\caption{Overall agreement of models with different settings weighted by task \mb{Change naming convention as main table gets updated}}
%\vspace*{-1em}
%\label{fig:overall_agreement}
%\end{figure}


% However, we leave this line of investigation for other applications for future work. 

%We find that our model (att\_mt\_uqa) has the highest agreement with uqa\_mt (83.3\%). This validates that prompt transfer with pre-trained backbone model on source tasks helps to achieve similar model behavior to model tuning with 2500x fewer parameters. On the contrary, we find least agreement with pt-random which is intuitive. With the model performance results from Table 9 \mb{Reference missing in main table} and higher agreement scores with unified fine tuned model, it is derivable that prompt transfer essentially helps over vanilla prompt tuning with random or other heuristic initialization approaches. Another higher agreement scores between init-squad and init-format is due to the representative dataset for extractive QA in init-format is SQuaD. Extractive QA datasets cover 25\% of target datasets; hence we expect higher overlap in the results for init-squad and init-format. \par
%Fine-tuning separate models for each downstream task has the highest overlap of 85.1\% with a single unified model when pre-trained with our source tasks. The agreement score higher than t5-base single model (85.1\% v/s. 82\%) further validates the pre-training backbone helps achieve closer model behavior to fine-tune multiple models on each task. Additionally, more than 50\% of our source and target tasks have similar reasoning skills. Thus, we hypothesize that prompt transfer can be beneficial and achieve performance similar to fine-tuning with a higher overlap of skills between the source and target tasks. 

%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{Figs/heatmap_complentary.png}
%\vspace*{-2em}
%\caption{Heatmap showing gains from adjoining decisions between two models. \mb{Change naming convention as main table gets updated}}
%\vspace*{-1em}
%\label{fig:overall_complementary}
%\end{figure}



%\par \textbf{Analysis on complementary models:} 
%Figure~\ref{fig:overall_complementary} shows overall accuracy by unionizing model predictions from two settings. We see that having different initializations in prompt tuning helps overall performance. Interestingly, att\_mt\_uqa gains with 8.5\% when combined with init-format. On further analysis at task level, we find significant gains from different initializations to benefit tasks such as COPA, ReClor, Qualrel that underperformed individually in comparison with fine-tuning methods. We also find that combining models with different backbone models also leads to significant performance improvements across both fine-tuning and prompt-tuning settings. 

